Muskits-ESPnet: A Comprehensive Toolkit for Singing Voice Synthesis in New Paradigm

This research presents Muskits-ESPnet, a versatile toolkit that introduces new paradigms to Singing Voice Synthesis (SVS) through the application of pretrained audio models in both continuous and discrete approaches. Specifically, we explore discrete representations derived from SSL models and audio codecs and offer significant advantages in versatility and intelligence, supporting multi-format inputs and adaptable data processing workflows for various SVS models. The toolkit features automatic music score error detection and correction, as well as a perception auto-evaluation module to imitate human subjective evaluating scores. Muskits-ESPnet is available at \url{https://github.com/espnet/espnet}.

==> sec-exp.tex <==
\section{Experiments}
\label{sec:exp}

\begin{table}[!t]
\caption{\small Dataset. }%Details can be found in Section~\ref{ssec: transfer}.}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\textbf{Dataset} & \textbf{language} & \textbf{singer} & \textbf{scale} \\
\midrule
Opencpop & zh &  &   \\
Ofuton & jp &  &  \\
CSD & en/kr & & \\
ACE-Opencpop  & zh &  &  \\
... & & & \\
\bottomrule
\end{tabular}
}
\label{tab: transfer}
\end{table}

\subsection{Comparison of other SVS toolkits}

\begin{table}[!t]
\caption{\small Comparison with other toolkits.}%Details can be found in Section~\ref{ssec: transfer}.}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\textbf{Toolkit} & \textbf{Datasets} & \textbf{Models} & \textbf{languages} \\
\midrule
sys1    &   &  &  \\
sys2    &   &  &   \\
Muskits-v1 &  &  &   \\
Muskits-ESPnet & &   &  \\
\bottomrule
\end{tabular}
}
\label{tab: transfer}
\end{table}

\subsection{SVS results from different systems}

\begin{table}[!t]
\caption{\small }
\vspace{-8pt}
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c|ccccc|c}
\toprule
\textbf{Representation} & \textbf{MCD ↓} & \textbf{F0 ↓}  & \textbf{SA ↑} & \textbf{VUV} & \textbf{MOS ↑}  \\
% \textbf{Representation} & \textbf{MCD ↓} & \textbf{F0 ↓}  & \textbf{SA ↑} & \textbf{Pron ↑} & \textbf{Melody ↑} & \textbf{Tech ↑} & \textbf{MOS ↑} & \textbf{Dimension} \\
\midrule
Mel NAR & 8.00 & 0.19 & 59\% &  & 3.42 \\
Mel seq2seq & & & & & \\
Mel AR & & & & & \\
Mel JT & & & & & \\
\midrule
Latent variance  & 7.76  & 0.18 & \textbf{62\%} &  & 3.68  \\
Discrete token & \textbf{7.56} & \textbf{0.17} & \textbf{61\%} &   & \textbf{3.70} \\
\midrule
GT & - & - & - & & 4.59  \\
\bottomrule
\end{tabular}
}
\label{tab: comparison}
\end{table}

\subsection{Multi Singer and Transfer Learning}

\begin{table}[!t]
\caption{\small Transfer learning from multi singer dataset ACE-Opencpop to single singer dataset Opencpop. }%Details can be found in Section~\ref{ssec: transfer}.}
\centering
\resizebox{1\columnwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
% \textbf{Representation} & \textbf{MCD ↓} & \textbf{F0 ↓} & \textbf{MOS ↑} \\
\begin{tabular}{c|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Representation}} & \multicolumn{2}{c|}{\textbf{Vocoder}} & \multicolumn{2}{c}{\textbf{+ Acoustic}} \\
% \cline{2-5}
 & \textbf{MCD ↓} & \textbf{F0 ↓}  & \textbf{MCD ↓} & \textbf{F0 ↓}  \\
\midrule
ACE-Opencpop    & \textbf{5.60}  & \textbf{0.14} & - & - \\
Opencpop-origin & 6.51 & 0.16 & 8.15 & 0.19 \\
Opencpop-transfer & 6.11 & 0.16 & \textbf{7.43} & \textbf{0.17} \\
\bottomrule
\end{tabular}
}
\label{tab: transfer}
\end{table}

\subsection{Task Combination}
